Do Energy-oriented Changes Hinder Maintainability?

Energy efficiency is a crucial quality requirement for mobile applications. However, improving energy efficiency is far from trivial as developers lack the knowledge and tools to aid in this activity. In this paper we study the impact of changes to improve energy efficiency on the maintainability of Android applications. Using a dataset containing 539 energy efficiency-oriented commits, we measure maintainability -- as computed by the Software Improvement Group's web-based source code analysis service Better Code Hub (BCH) -- before and after energy efficiency-related code changes. Results show that in general improving energy efficiency comes with a significant decrease in maintainability. This is particularly evident in code changes to accommodate the Power Save Mode and Wakelock Addition energy patterns. In addition, we perform manual analysis to assess how real examples of energy-oriented changes affect maintainability. Our results help mobile app developers to 1) avoid common maintainability issues when improving the energy efficiency of their apps; and 2) adopt development processes to build maintainable and energy-efficient code. We also support researchers by identifying challenges in mobile app development that still need to be addressed.

==> Makefile <==
REVISION=288df0cc981636900dfaa00de4297ca31568206f
PANDOC_PDFOPTIONS = -f markdown+link_attributes+inline_notes --variable fontsize=10pt \
						 --variable papersize=a4 --variable geometry:margin=1in --reference-links \
             --variable documentclass=article \
						 -H quote-setup.tex


pdf:
	latexmk -pdf paper

rtf:
	latex2rtf -M4 paper
	echo "Open master.rtf with Word. Make the necessary changes and convert to docx (File > Convert document..)"
	echo "Then convert to epub:  /Applications/calibre.app/Contents/MacOS/ebook-convert master.docx master.epub"

# Usage: make diff [REVISION=commit_sha1]
diff:
	#git show $(REVISION):./master.tex > old.tex
	latexdiff submitted_1.tex paper.tex > diff.tex
	latexmk -pdf diff.tex
	latexmk -c diff.tex
	rm diff.tex

notes: $(wildcard *.md)
		$(foreach md_file, $?, pandoc $(md_file) $(PANDOC_PDFOPTIONS)  -o $(patsubst %.md, %.pdf, $(md_file));)
	

clean:
	latexmk -c


==> lifespan.tex <==

\newrquestion{rq:timespan}{How does the lifespan of energy efficiency-oriented commits compare to regular commits?}

\why{We want to understand whether energy-oriented changes are easy to
implement, without requiring extra effort from developers to maintain the code
introduced with those changes. Ideally, energy commits should not require
to be changed earlier than regular commits.}

\how{We look at the lifespan of energy commits: the time difference
between an energy-oriented commit and the first future commit that intersects
at least with one line of code. We apply the same procedure to general-purpose
commits and compare the results.}

\finding{Energy commits are more likely to be changed in the future than
regular commits. In addition, results show evidence that energy changes are
more difficult to implement than regular changes.}

\section{Methodology} \label{sec:methodology}

\subsection{Lifespan of Energy Commits}

We measure the lifespan of energy commits as the time in which an energy commit
lives in a project without being refactored. We do that by identifying the
first commit introduced after the energy commit that changes at least one line
of the energy commit (ignoring whitespaces), as depicted in
Fig.~\ref{fig:lifespan}. We refer to this new commit as the \textbf{refactoring
commit}. The lifespan is measured as the time difference between the energy
commit and the refactoring commit.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/commit_lifespan}
  \caption{Lifespan of a given energy commit.}
  \label{fig:lifespan}
\end{figure}

Although we use a simplistic approach to identify a refactoring commit: there
might be cases in which the developer simply changed a line in the
documentation. However, classifying the nature of the changes in the commit is
not a trivial task~\cite{pascarella2018self,da2017framework}. Instead, we
analyze the difference between the lifespan of \textbf{energy commits} and
\textbf{baseline commits}.

Finally, we perform the Kolmogorov-Smirnov test to reject the null hypothesis
that the lifespan of energy commits has the same distribution of the lifespan
of regular commits using a significance level of $\alpha=0.05$.

\section{Results}

\rquestion{rq:timespan}

The lifespan of energy commits in an Android project is depicted in
Fig.~\ref{fig:refactoring_timedelta}. The plot shows the distribution of the
lifespan in seven bins: 0--1h, 1h--1d, 1w--4w, 4w--1y, above 1 year, and one
last bin, \emph{Not changed}, counting energy commits that were never
refactored. The lifespan for energy commits is plotted in blue bars. In gray,
with dashed lines, is the lifespan distribution for the baseline. Energy
commits significantly differ from baseline commits in bins 0--1h and \emph{Not
changed}. Within the first hour after the commit, \textbf{23.1\% of energy
commits are refactored. This is considerably higher than the baseline}, which
reports 15.2\% of the cases. Moreover, 9.6\% of energy commits are not observed
to require further changes -- this is considerably lower than the baseline,
which reports 19.0\% of regular commits. The hypothesis test Kolmogorov-Smirnov
validates the differences between regular and energy commits with a $p$-value
of 0.03, below the significance level ($\alpha < 0.05$).

This means that 1) energy commits are more likely to be changed again within the first hour after being committed, and 2) energy commits are more likely to be refactored than any other commit.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{../reports/refactoring_timedelta.pdf}
  \vspace{-0.4in}
  \caption{Distribution of the lifespan of energy-oriented commits.}
  \vspace{-0.2in}
  \label{fig:refactoring_timedelta}
\end{figure}

\section{Discussion}
\label{sec:discussion}

\rquestion{rq:timespan}

\emph{\textbf{Energy commits are more likely to be refactored than regular
commits. Moreover, refactorings are more likely to occur within the first
hour.}} These findings reinforce the importance of addressing maintainability
in energy-oriented changes: developers have to refactor the changes introduced
in these commits.

We do not study the nature of the refactorings performed, as they can occur due
to a number of reasons: bug fixes, code cleaning, changes in APIs, addition of
new features, etc. However, the fact that they have a different lifespan than
the baseline shows that energy commits entail challenges that have not been
addressed yet by the community.

The fact that energy commits are more likely to change within the first hour
can be seen as an indicator of the difficulty of implementing energy-saving
features. Developers struggle to implement these features, incurring to new
refactoring commits before reaching a stable implementation.

Future work should focus on analyzing the timeline of energy commits. I.e.,
analyzing not only the first refactoring commit, classify the purpose of the
refactor. This work could be extended beyond the domain of energy-oriented
changes, including security commits, user experience improvements, storage
management, etc. However, designing a reliable automated approach is still an
open problem~\cite{da2017framework,sliwerski2005changes,pascarella2018self}.

\section{Threats to Validity}
\label{sec:t2v}

The lifespan of a given energy commit is an approximation based on a single
change in one of the lines of code submitted by that commit. Although changes in
whitespace are not considered, we did not perform any evaluation on the type of
change that is performed. Some changes may be trivial while others may have
required more efforts from developers. Related work has proposed approaches to
automatically classify changes (e.g., bug fixes\cite{da2017framework}, and
refactorings~\cite{pascarella2018self}), but we have not explored them.
Nevertheless, we understand that the differences in the lifespan between our
dataset of energy changes and the baseline provide interesting leads for
discussion and new research directions.
